Exploring Temporal Dependencies in Multimodal Referring Expressions with Mixed Reality

In collaborative tasks, people rely both on verbal and non-verbal cues simultaneously to communicate with each other. For human-robot interaction to run smoothly and naturally, a robot should be equipped with the ability to robustly disambiguate referring expressions. In this work, we propose a model that can disambiguate multimodal fetching requests using modalities such as head movements, hand gestures, and speech. We analysed the acquired data from mixed reality experiments and formulated a hypothesis that modelling temporal dependencies of events in these three modalities increases the model's predictive power. We evaluated our model on a Bayesian framework to interpret referring expressions with and without exploiting a temporal prior.

==> methods_old.tex <==
\section{Methodology}

\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth,scale=0.5]{observation_update3.jpg}
\caption{Observation update with a temporal prior (TODO: change g to h)}
\label{fig:observation}
\end{figure}

\subsection{Bayesian Filter}

Having three continuous modalities, we want to fuse them together in order to get a probability distribution over all objects ($\mathcal{X}$), given observed speech, head, and pointing inputs ($\mathcal{Z}$) at each time step ($t$). We apply probabilistic inference based on Bayesian filtering \cite{thrun2005probabilistic}. The hidden state, $x_t \in \mathcal{X}$, is the target object in the scene that the person is currently referencing. The robot observes the user's non-verbal actions and speech, $\mathcal{Z}$, and at each time step estimates a distribution over the current state, $x_t$:

\begin{equation}
p(x_t|z_{0:t})
\end{equation}

First, a prediction about current state is made based only on previous observations and then two types of update are made: time update without any contextual information and observation update, as proposed in \cite{whitney2016interpreting}.

\subsection{Observation update}

The posterior distribution of $x_t$ given the present and all past observations, $z_{0:t}$, is obtained using the Bayesian rule:

\begin{equation}\label{obs-eq}
p(x_t|z_{0:t}) = \frac{p(z_t|x_{t})\times p(x_{t}|z_{0:t-1})}{p(z_{t}|z_{0:t-1})} \propto p(z_t|x_{t})\times p(x_{t}|z_{0:t-1})
\end{equation}

The observation model calculates the probability of the observation given the state. Each observation is a set of the user's head movement, hands pointing, and speech, $<h, l, r, s>$ where:
\begin{itemize}
	\item $h$ represents a 3D vector of angular velocities from head movements.
    \item $l$ represents a 3D vector of angular velocities from the user's left hand index finger.
    \item $r$ represents a 3D vector of angular velocities from the user's right hand index finger.
    \item $s$ represents the observed speech from the user, consisting of a list of words.
\end{itemize}

More formally, the observation model looks as follows:

\begin{equation}
p(z_t|x_{t}) = p(h, l, r, s|x_t)
\end{equation}

We factor our observations assuming that each modality is conditionally independent of the others given the target object. In other words, we are assuming that if we know the true target object, the probabilities of the user pointing at that object with their left hand or right, head movements are conditionally independent:

\begin{equation}
p(z_t|x_{t}) = p(h | x_t) \times p(l | x_t) \times p(r | x_t) \times p(s | x_t)
\end{equation}

\subsubsection{Head Movement}\label{head}

Our approach here is to create a model that translates head movements into gaze direction. We want to have coordinates of where the person is looking at given their head angular velocities and the distance from the table. A naive model is to project a vector from the centre of human's head onto the shared workspace. The problem with this approach is that head movements have a lesser amplitude compared to eye movements. We solve it by performing calibration first. Following the guidelines for an eye tracker calibration \cite{harezlak2014towards}, we train a Support Vector Regression (SVR) \cite{smola2004tutorial} with a RBF kernel (C=10, gamma=5) on 14 points augmented in the workspace. Each point is displayed for the total duration of 1950 ms, out of which the first 700 ms are ignored in the training process. 

% If a fixation is detected in the stream of angular velocities from head movements, then we combine all normalized angular velocities into a vector h = (hx, hy, hz). 

% To obtain an estimate of the gaze direction, we want to find a mapping
% SVR x : f(head angular velocity x, y, z, distance to the table) -> g(x)
% SVR y : f(head angular velocity x, y, z, distance to the table) -> g(y)

The calibration process gives us a $5\pm1.89$ cm, while the naive approach performs at $63\pm20.75$ cm error rate.

In order to translate coordinates acquired from the $SVR_h$ into a probability distribution over all objects, we use a Gaussian kernel ($\mathcal{N}$) with variance ($\mathcal{\sigma}$) around the predicted gaze point. We define a function  $D(o, x)$ as distance between the predicted gaze point from $SVR_h$, $o$, and the centre of mass of object $x$:

\begin{equation}
p(h|x_{t}) \propto \mathcal{N}(\mu_h=0, \sigma_h)[D(h, x_t)]
\end{equation}

\subsubsection{Gestures}

Pointing detection is made with the help of LeapMotion API. The calibration process afterwords follows the same steps as \ref{head} for each hand separately, learning $SVR_l$ and $SVR_r$. As a result, the gesture model is computed as distance between the centre of mass of object $x$ and a predicted coordinates of pointing on the table weighted by a Gaussian kernel:

\begin{equation}
p(l|x_{t}) \propto \mathcal{N}(\mu_l=0, \sigma_l)[D(l, x_t)]
\end{equation}
\begin{equation}
p(r|x_{t}) \propto \mathcal{N}(\mu_r=0, \sigma_r)[D(r, x_t)]
\end{equation}

\subsubsection{Speech}

As with the other modalities, first we use speech recognition to convert audio to text and then perform keywords dictionary-based classification to identify the following speech events: 

\begin{itemize}
    \item attribute - adjectives that describes size, shape or colour of a Lego block from the workspace, e.i. \textit{red, large, cylinder}, etc.
    \item deictic - e.i. \textit{here, there, this, that}, etc.
    \item other - any other word that is not included into the previous two categories
\end{itemize}

As an extra speech event, the beginning of a verbal request is detected from the audio directly. These specific classes  were inferred from the initial data collection. The highest correlation was shown between them and events in other modalities.

After detecting speech events, we represent it with a unigram model. Namely, we take each word $w$ in a given speech input $s$ and calculate the probability that, given state $x_t$, that word would have been spoken.

\begin{equation}
p(s|x_{t}) = \displaystyle\prod_{w\in s} p(w|x_t)
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% THE FOLLOWING IS UNDER CONSTRUCTION %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Temporal Priors}

The main hypothesis of this paper, is whether incorporating the knowledge of temporal relationships between high-level events in the input modalities can increase performance of the Bayesian filter. Thus, we introduce temporal priors to the observation update, equation \ref{obs-eq}, as follows:

\begin{equation}\label{obs-temp-eq}
p(x_t|z_{0:t}) \propto p(z_t|x_{t})\times p(x_{t}|z_{0:t-1}) \times p(z_t), 
\end{equation}

where $p(z_t)$ is a temporal prior and can be represented as:

\begin{equation}
p(z_t) = p(h,l,r,s)
\end{equation}

We define a temporal prior as a joint temporal probability distribution of events happening in one modality during a certain time interval given events in other modalities. In other words, temporal priors can encode, for example, that if a person said "this", the probability of them pointing at the intended object a second before this event rises dramatically.

First, we employ definition, formulated in \cite{kwon2012temporal}, of temporal probability of event $X=x_i$ starting at time $T_X$ and occurring during a time interval between $t_1$ and $t_1$ given an observed event $Y=y_j$ at time $T_Y=t_y$, as

\begin{equation}\label{eq:condTimeProb}
	\begin{multlined}
p(X=x_i, t_1 \leq T_X \leq t_2 | Y=y_j, T_Y = t_y) =
\\= p(X=x_i| Y=y_j) \times p(t_1 \leq T_X \leq t_2 | T_Y = t_y, Y=y_i, X=x_i) =
\\= p(X=x_i| Y=y_j) \times \int_{t_1}^{t_2} f_{Z_{ij}}(t_x-t_y)dt_y
	\end{multlined}
\end{equation}

"Where $Z_{ij}$ is a temporal random variable of the time-interval between $T_X$ and $T_Y$ given $X=x_i$ and $Y=y_j$, and $f_{Z_{ij}}$ is a PDF of $Z_{ij}$." For our intents and purposes, only temporal probability is of interest. Thus, we assume that all events have an equal probability to happen and equation \eqref{eq:condTimeProb} will be as follows

\begin{equation}\label{eq:condTimeProbTwo}
	\begin{multlined}
p(X=x_i, t_1 \leq T_X \leq t_2 | Y=y_j, T_Y = t_y) \propto \int_{t_1}^{t_2} f_{Z_{ij}}(t_x-t_y)dt_y
	\end{multlined}
\end{equation}

In this paper, multivariate Gaussian Mixture Models (GMMs) are used to represent the PDF of $f_{Z_{ij}}(t_x-t_y)$. We assume that modalites are temporally dependent; thus, the covarience matrix is learned alongside kernels' means. We train GMMs with an Expectation Maximisation (EM) algorithm. Online adaptation of the model is performed via Maximum A Posteriori (MAP) estimation approach, as in Reynolds' work \cite{reynolds2000speaker}, due to a limited number of samples that we are able to collect during the interaction.

% I want to talk about the noisiness of head movement and accuracy, while speech gives less information but is a less noissy modality in a sence that we are better at controlling speech then, for instance, head movements. But I think I've written it already somewhere. 

Since our goal is to exploit modalities that give more information and are faster at providing cues which object is the target one (gestures, head movements), we use speech as the base modality due to it's relatively low level of nosiness. As a data pre-processing step, time intervals are computed between events closest to the closest events in the speech modality. 

%All in all, temporal priors are used to highlight fixations on the target object based on the relative time interval between the fixation and. 



% We found the most frequent informative sequences of events and computed time intervals to the nearest speech events. The acquired distributions of time intervals were tested on significance and modelled using Gaussian Mixture Models (GMMs). %\cite{marin2005bayesian}. 
% The fitted GMMs were later used as temporal priors in a Bayesian filter, that encoded a probability distribution of an object being the target object given current and previous multimodal input. The effectiveness of temporal priors was evaluated on accuracy and decision making time. 


